Blockchain Privacy Through Merge Avoidance and Mixing Services: a Hardness and an Impossibility Result

Cryptocurrencies typically aim at preserving the privacy of their users. Different cryptocurrencies preserve privacy at various levels, some of them requiring users to rely on strategies to raise the privacy level to their needs. Among those strategies, we focus on two of them: merge avoidance and mixing services. Such strategies may be adopted on top of virtually any blockchain-based cryptocurrency. In this paper, we show that whereas optimal merge avoidance leads to an NP-hard optimization problem, incentive-compatible mixing services are subject to a certain class of impossibility results. Together, our results contribute to the body of work on fundamental limits of privacy mechanisms in blockchain-based cryptocurrencies.

==> adicionais.tex <==

\subsection{Explorações adicionais}

Como resultado do \emph{nao-previne}, precisamos explorar alternativas para conferir ao DiCent a prevenção de ambas as formas de \emph{Edge Insertion}. Uma possibilidade é utilizar o DiCent da forma atual, que previne o ataque apenas quando realizado por nós intermediários, e impedir um ataque pelo nó destino pelo projeto do protocolo. Isto pode ser feito, por exemplo, conferindo ao último nó intermediário (isto é, o nó que faz a entrega da mensagem diretamente ao destinatário) a responsabilidade de reportar esta entrega.

Outra possibilidade é a de modificar o DiCent para que ele deixe de possuir alguma das características exigidas por hipótese no \emph{nao-previne}.  Dentre elas, a ausência da propriedade (\ref{zero-sum}) parece ser a possibilidades mais interessante de se explorar, visto que as demais são facilmente justificadas por princípios de projeto no estilo `navalha de Occam'.

A propriedade (\ref{zero-sum}) nos diz que o mecanismo não interfere no total de créditos presentes no sistema ao realizar cobranças e recompensas: todos os créditos cobrados do destinatário são distribuídos entre os nós intermediários segundo alguma regra (por exemplo, igualmente entre todos eles). A forma mais simples de incorporar isto ao DiCent é dividir o total de créditos cobrados do nó destino em duas componentes, uma a ser distribuída em forma de recompensa e outra a ser incorporada ao total presente no sistema. Chamaremos esta segunda componente de \emph{taxa}.

Para formalizar, utilizaremos uma notação semelhante à descrita na prova do \emph{nao-previne}: para uma mensagem que percorre uma rota $\mathcal{R}$ de comprimento $l$, denotemos por $R(l)$ a recompensa a ser recebida por cada nó intermediário, e $T(l)$ a taxa adicional a ser cobrada do nó destinatário. O total de créditos que o nó destinatário deverá pagar é dado por $C(l) = l\cdot R(l) + T(l)$.

Da mesma forma, seja $AI(l,k)$ e $AD(l,k)$ a vantagem em créditos obtida por um atacante intermediário e um atacante destinatário, respectivamente, ao realizar um ataque de \emph{Edge Insertion} de tamanho $k$ (isto é, adicionar $k$ nós sybil) em uma rota de tamanho original $l$. Como a taxa não interfere com a recompensa a ser recebida, a expressão para $AI(l,k)$ permanece igual ao caso anterior: $$AI(l,k) = (k+1)\cdot R(l+k).$$ No entanto, a expresão para $AD(l,k)$ será modificada: $$AD(l,k) = C(l+k) - k\cdot R(l+k) = l\cdot R(l+k) + T(l+k).$$

As condições para prevenção dos dois tipos de ataque permanecem: para qualquer $k > 0$ e qualquer $l$, $AI(l,k) \leq AI(l,0)$ e $AD(l,k) \geq AD(l,0)$. Estas condições se traduzem nas seguintes desigualdades:

\begin{align}
(k+1)\cdot R(l+k) &\leq R(l)\label{condicao-ei-intermediario}\\
l\cdot R(l+k) + T(l+k) &\geq l\cdot R(l) + T(l)\label{condicao-ei-destinatario}
\end{align}

Nosso objetivo, então, é determinar quais funções $R(\cdot)$ e $T(\cdot)$ satisfazem estas desigualdades, além da desigualdade adicional $R(\cdot) > 0$ (para que não se degenere a recompensa a ser paga aos nós destinatários). Qualquer solução para este sistema nos diz quanto devemos cobrar do nó destinatário e quanto devemos distribuir de recompensa a cada nó intermediário para que ambas as formas do ataque de \emph{Edge Insertion} sejam desencorajadas.

Para resolver este problema, começamos simplificando nossas condições aplicando o seguinte resultado:

\begin{lemma}
Sejam $R(\cdot)$ e $T(\cdot)$ funções reais sobre $\mathbb{N}$, sendo $R(\cdot)>0$. Se $R(\cdot)$ e $T(\cdot)$ satisfazem (\ref{condicao-ei-intermediario}) e (\ref{condicao-ei-destinatario}) para $k = 1$ e todo $l\in\mathbb{N}$, então satisfazem (\ref{condicao-ei-intermediario}) e (\ref{condicao-ei-destinatario}) para todo $k,l\in\mathbb{N}$.
\end{lemma}

\begin{proof}
A prova segue por indução completa no valor de $k$, com a base de indução sendo a própria hipótese do lema. Suponha que a hipótese de indução completa seja verdadeira, isto é, que para todo $k'\in\mathbb{N}, k'<k$ e $l\in\mathbb{N}$:

\begin{align*}
(k'+1)\cdot R(l+k') &\leq R(l) \\
l\cdot R(l+k') + T(l+k') &\geq l\cdot R(l) + T(l)
\end{align*}

Queremos mostrar que valem:

\begin{align*}
(k+1)\cdot R(l+k) &\leq R(l) \\
l\cdot R(l+k) + T(l+k) &\geq l\cdot R(l) + T(l)
\end{align*}

Para a primeira condição, temos que:
$$R(l+k) \leq \frac{R(l+k-1)}{2}
\leq \frac{R(l)}{2k}
\leq \frac{R(l)}{k+1},$$
onde as duas primeiras desigualdades seguem da hipótese de indução (com parâmetros $l+k-1$ e $1$, e $l$ e $k-1$, respectivamente) e a última desigualdade segue do fato de que $k \geq 1$.

Para a segunda condição, temos que:
\begin{align*}
l\cdot R(l) + T(l) &\leq l\cdot R(l+1) + T(l+1) \\
&= (l+1)\cdot R(l+1) + T(l+1) - R(l+1) \\
&\leq (l+1)\cdot R(l+k) + T(l+k) - R(l+1) \\
%&= (l+k) \cdot R(l+k) + T(l+k) - R(l+1) - (k-1)\cdot R(l+k) \\
&\leq (l+k) \cdot R(l+k) + T(l+k),
\end{align*}
onde novamente utilizamos nas duas primeiras desigualdades a hipótese de indução (com parâmetros $l$ e $1$, e $l+1$ e $k-1$, respectivamente) e, na última, o fato de $R(\cdot)$ ser uma função positiva. Isto conclui a prova.
\end{proof}

Este resultado nos garante que basta encontrar funções $R(\cdot)$ e $T(\cdot)$ satisfazendo as desigualdades simplificadas:
\begin{align*}
2R(l+1) &\leq R(l)\\
l\cdot R(l+1) + T(l+1) &\geq l\cdot R(l) + T(l),
\end{align*}
além da desiguldade adicional $R(\cdot) > 0$. Implicitamente, o resultado que usamos diz que desencorajarmos o ataque de \emph{Edge Insertion} em sua forma mais simples ($k=1$ nó sybil), também conseguiremos desencorajar ataques com mais nós sybil.

Podemos determinar uma fórmula geral para as soluções deste sistema de inequações olhando para as equações correspondentes:
\begin{align*}
2R(l+1) &= R(l)\\
l\cdot R(l+1) + T(l+1) &= l\cdot R(l) + T(l),
\end{align*}
que podem ser vistas como um caso limítrofe do sistema de inequações. As soluções deste sistema são dadas por:
\begin{align*}
R(l) &= R(1)\cdot 2^{-l+1} \\
T(l) &= T(1) + \mathcal{S}(l)R(1), \\
\end{align*}
onde $R(1) > 0$ e $T(1)$ são constantes e $\mathcal{S}(l) = \sum_{j=1}^{l-1} j2^{-j} = 2-(l+1)2^{-l+1}$. Disto, derivamos a solução geral do sistema de inequações: % TODO: mudar definição de S(l) para usar S(l) em vez de S(l-1) (implicações na definição abaixo)

\begin{theorem}
Sejam constantes reais $R_0 > 0$ e $T_0$ e funções $\rho,\tau:\mathbb{N}\to\mathbb{R}$ não-negativas com $\rho(\cdot)$ não-crescente e $\tau(\cdot)$ não-decrescente. Defina:
\begin{align*}
R(l) &= R_0 \cdot 2^{-l+1}\rho(l) \\
T(l) &= T_0 + R_0\cdot\mathcal{S}(l) + \sum_{i=1}^{l-1}[\rho(i)-\rho(l)] + \tau(l) %TODO: reformular com rho multiplicativo
\end{align*}

Então $R(\cdot) > 0$, e $R(\cdot)$ e $T(\cdot)$ satisfazem (\ref{condicao-ei-intermediario}) e (\ref{condicao-ei-destinatario}) para todo $k,l\in\mathbb{N}$.\label{solucoes}
\end{theorem}

% TODO: provar este teorema

O \emph{solucoes} nos dá uma fórmula geral para as funções recompensa $R(\cdot)$ e taxa $T(\cdot)$, na qual temos liberdade para escolher duas constantes $R_0$ e $T_0$, e duas funções $\rho$ e $\tau$. De maneira geral, gostaríamos de realizar escolhas que nos garantam que $R(l)$ e $T(l)$ sejam números inteiros positivos para comprimentos de rota $l$ suficientemente curtos. Isto facilita a implementação de protocolos baseados nesta generalização do DiCent.

No entanto, devemos discutir com mais detalhes a escolha de $T_0$ em particular, devido às suas implicações na economia da rede. Como discutimos anteriormente, a cobrança de uma taxa adicional ao nó destinatário, como forma de desencorajar ataques de \emph{Edge Insertion} por parte do nó destinatário, não é uma solução desejada pois tem a tendência de remover créditos do sistema. No entanto, a descrição da solução geral dada pelo \emph{solucoes} nos permite, exclusivamente pela escolha de $T_0$, projetar soluções tais que $T(l) < 0$ para valores de $l$ suficientemente baixos.

Uma interpretação natural de tais soluções é que, para mensagens cujo comprimento de rota $l$ satisfaz $T(l) < 0$, o sistema está na realidade inserindo créditos na rede, ao cobrar do nó destinatário um total de créditos menor do que será distribuído aos nós intermediários, assim ``financiando'' o roteamento através de tais rotas. Caso conheçamos a distribuição do comprimentos das rotas atravessadas pelas mensagens, podemos escolher um valor de $T_0$ tais que o número total de créditos no sistema permaneça, em média, constante.

